Simple Extensions of Polytopes

We introduce the simple extension complexity of a polytope P as the smallest number of facets of any simple (i.e., non-degenerate in the sense of linear programming) polytope which can be projected onto P. We devise a combinatorial method to establish lower bounds on the simple extension complexity and show for several polytopes that they have large simple extension complexities. These examples include both the spanning tree and the perfect matching polytopes of complete graphs, uncapacitated flow polytopes for non-trivially decomposable directed acyclic graphs, hypersimplices, and random 0/1-polytopes with vertex numbers within a certain range. On our way to obtain the result on perfect matching polytopes we generalize a result of Padberg and Rao's on the adjacency structures of those polytopes. To complement the lower bounding techniques we characterize in which cases known construction techniques yield simple extensions.

==> TikZ-extended-formulations-bicliques.tex <==
\piDeclareString{job}{}
\piDeclareBool{colors}{true}
\piDeclareBool{decorations}{true}

\piParse % Parses all given options

\piIfString{job}{config}{%
  % Preamble code
  \usetikzlibrary{fadings}
  \usetikzlibrary{shapes.geometric}
}{
  \piIfString{job}{face-vertex-biclique}{
    \tikzset{
      circleStyle/.style={circle,inner sep=1.0mm},
      rectStyle/.style={rectangle,inner sep=1.2mm},
      starStyle/.style={star,star point height=2pt,inner sep=0.7mm},
      incidence/.style={thin,gray}
    }

    \piIfBool{colors}{
      \tikzset{
        faceStyle/.style={thick,draw=black,fill=white},
        bclFaceStyle/.style={thick,draw=black,fill=blue},
        bclGeneratorStyle/.style={very thick,draw=red,fill=blue},
        bclVertexStyle/.style={thick,draw=black,fill=green!70!black}
      }
    }{
      \tikzset{
        faceStyle/.style={thick,draw=black,fill=white},
        bclFaceStyle/.style={thick,draw=black,fill=gray},
        bclGeneratorStyle/.style={thick,draw=black,fill=black},
        bclVertexStyle/.style={thick,draw=black,fill=gray}
      }
    }

    % draw a fading ray from (#1,#2) of degree #3 with fading in #4
    \def\fadingRay#1#2#3#4{
      \node (foo) at (#1,#2) {};
      \draw[draw=none,fill=gray,path fading=#4,rotate=#3] (foo) rectangle +(0.01,0.6);
    }
    \def\fadingNorthRay#1#2#3{\fadingRay{#1}{#2}{#3}{north}}
    \def\fadingSouthRay#1#2#3{\fadingRay{#1}{#2}{#3}{south}}

    % border frame
    \draw[thick,fill=white!95!black]
      (1.25,-0.3) ..controls(1.15,-0.3)..
      (1.15,-0.2) ..controls(1.15,0.2)..
      (1.4,0.7) ..controls(1.5,0.9)and(1.8,0.9)..
      (1.9,1.1) -- 
      (2.2,3.0) ..controls(2.2,3.1)and(2.35,3.2).. 
      (2.4,3.3) ..controls(2.6,4.0)..
      (2.8,4.0) -- 
      (3.7,4.0) ..controls(3.9,4.0)..
      (4.1,3.3) ..controls(4.2,3.1)..
      (4.2,3.0) -- 
      (4.3,1.8) ..controls(4.35,1.65)and(4.65,1.7)..
      (4.7,1.6) ..controls(5.35,0.2).. 
      (5.35,-0.2) ..controls(5.35,-0.3)..
      (5.25,-0.3) -- 
      cycle;

    % positions
    \def\vax{-0.2}  \def\vay{0}   \def\va{(\vax,\vay)}
    \def\vbx{0.3}   \def\vby{0}   \def\vb{(\vbx,\vby)}
    \def\vcx{0.8}   \def\vcy{0}   \def\vc{(\vcx,\vcy)}
    \def\vdx{1.5}   \def\vdy{0}   \def\vd{(\vdx,\vdy)}
    \def\vex{2.0}   \def\vey{0}   \def\ve{(\vex,\vey)}
    \def\vfx{2.5}   \def\vfy{0}   \def\vf{(\vfx,\vfy)}
    \def\vgx{3.0}   \def\vgy{0}   \def\vg{(\vgx,\vgy)}
    \def\vhx{3.5}   \def\vhy{0}   \def\vh{(\vhx,\vhy)}
    \def\vix{4.0}   \def\viy{0}   \def\vi{(\vix,\viy)}
    \def\vjx{4.5}   \def\vjy{0}   \def\vj{(\vjx,\vjy)}
    \def\vkx{5.0}   \def\vky{0}   \def\vk{(\vkx,\vky)}
    \def\vlx{5.7}   \def\vly{0}   \def\vl{(\vlx,\vly)}
    \def\vmx{6.2}   \def\vmy{0}   \def\vm{(\vmx,\vmy)}

    \def\eax{1.75}  \def\eay{0.7} \def\ea{(\eax,\eay)}
    \def\ebx{2.75}  \def\eby{0.7} \def\eb{(\ebx,\eby)}
    \def\ecx{4.75}  \def\ecy{0.7} \def\ec{(\ecx,\ecy)}

    \def\fax{4.5}   \def\fay{1.4} \def\fa{(\fax,\fay)}
    \def\fbx{2.5}   \def\fby{3.0} \def\fb{(\fbx,\fby)}
    \def\fcx{4.0}   \def\fcy{3.0} \def\fc{(\fcx,\fcy)}
    \def\fdx{0.5}   \def\fdy{2.0} \def\fd{(\fdx,\fdy)}
  
    \def\tax{2.75}  \def\tay{3.7} \def\ta{(\tax,\tay)}
    \def\tbx{3.25}  \def\tby{3.7} \def\tb{(\tbx,\tby)}
    \def\tcx{3.75}  \def\tcy{3.7} \def\tc{(\tcx,\tcy)}
    \def\tdx{1.5}   \def\tdy{3.7} \def\td{(\tdx,\tdy)}
    \def\tex{1.0}   \def\tey{3.7} \def\te{(\tex,\tey)}
    \def\tfx{0.5}   \def\tfy{3.7} \def\tf{(\tfx,\tfy)}
    \def\tgx{5.0}   \def\tgy{3.7} \def\tg{(\tgx,\tgy)}

    \def\P{(3.25,5.0)}
    \def\E{(3.25,-1.3)}

    % fading incidences - degrees 0 and 180 are buggy!
    \fadingNorthRay{\vax}{\vay}{0}     \fadingNorthRay{\vax}{\vay}{-30}   \fadingNorthRay{\vax}{\vay}{-60}
    \fadingNorthRay{\vbx}{\vby}{30}    \fadingNorthRay{\vbx}{\vby}{0}     \fadingNorthRay{\vbx}{\vby}{-30}
    \fadingNorthRay{\vcx}{\vcy}{30}    \fadingNorthRay{\vcx}{\vcy}{0}     \fadingNorthRay{\vcx}{\vcy}{-30}
    \fadingNorthRay{\vdx}{\vdy}{30}
    \fadingNorthRay{\vex}{\vey}{-10}   \fadingNorthRay{\vex}{\vey}{-30}
    \fadingNorthRay{\vfx}{\vfy}{30}    \fadingNorthRay{\vfx}{\vfy}{5}     \fadingNorthRay{\vfx}{\vfy}{-40}
    \fadingNorthRay{\vgx}{\vgy}{-5}    \fadingNorthRay{\vgx}{\vgy}{-30}
    \fadingNorthRay{\vhx}{\vhy}{30}    \fadingNorthRay{\vhx}{\vhy}{1}     \fadingNorthRay{\vhx}{\vhy}{-30}
    \fadingNorthRay{\vix}{\viy}{30}    \fadingNorthRay{\vix}{\viy}{1}     \fadingNorthRay{\vix}{\viy}{-30}
    \fadingNorthRay{\vjx}{\vjy}{30}    \fadingNorthRay{\vjx}{\vjy}{1}
    \fadingNorthRay{\vkx}{\vky}{40}
    \fadingNorthRay{\eax}{\eay}{40}    \fadingNorthRay{\eax}{\eay}{10}
    \fadingNorthRay{\ebx}{\eby}{30}    \fadingNorthRay{\ebx}{\eby}{1}     \fadingNorthRay{\ebx}{\eby}{-30}
    \fadingNorthRay{\ecx}{\ecy}{40}    \fadingNorthRay{\ecx}{\ecy}{-30}
    \fadingNorthRay{\fax}{\fay}{-10}   \fadingNorthRay{\fax}{\fay}{-40}   \fadingSouthRay{\fax}{\fay}{150}
    \fadingSouthRay{\fbx}{\fby}{160}   \fadingSouthRay{\fbx}{\fby}{180}   \fadingSouthRay{\fbx}{\fby}{200}
    \fadingSouthRay{\fcx}{\fcy}{150}   \fadingSouthRay{\fcx}{\fcy}{170}   \fadingSouthRay{\fcx}{\fcy}{190}
    \fadingNorthRay{\fdx}{\fdy}{1}     \fadingNorthRay{\fdx}{\fdy}{-30}
    \fadingSouthRay{\fdx}{\fdy}{150}   \fadingSouthRay{\fdx}{\fdy}{179}   \fadingSouthRay{\fdx}{\fdy}{210}
    \fadingSouthRay{\tax}{\tay}{210}
    \fadingSouthRay{\tbx}{\tby}{179}
    \fadingSouthRay{\tcx}{\tcy}{150}
    \fadingSouthRay{\tdx}{\tdy}{150}   \fadingSouthRay{\tdx}{\tdy}{179}   \fadingSouthRay{\tdx}{\tdy}{210}
    \fadingSouthRay{\tex}{\tey}{150}   \fadingSouthRay{\tex}{\tey}{179}   \fadingSouthRay{\tex}{\tey}{210}
    \fadingSouthRay{\tfx}{\tfy}{150}   \fadingSouthRay{\tfx}{\tfy}{179}   \fadingSouthRay{\tfx}{\tfy}{210}
    \fadingSouthRay{\tgx}{\tgy}{150}   \fadingSouthRay{\tgx}{\tgy}{179}   \fadingSouthRay{\tgx}{\tgy}{210}

    % create nodes
    \foreach \name/\coord in {va/\va, vb/\vb, vc/\vc, vl/\vl, vm/\vm} {
      \node[bclVertexStyle,starStyle] (\name) at \coord {};
    }
    \foreach \name/\coord in {vd/\vd, ve/\ve, vf/\vf, vg/\vg, vh/\vh, vi/\vi, vj/\vj,
        vk/\vk, eb/\eb, ec/\ec, fb/\fb, fc/\fc} {
      \node[bclFaceStyle,rectStyle] (\name) at \coord {};
    }
    \foreach \name/\coord in {ea/\ea, fa/\fa, ta/\ta, tb/\tb, tc/\tc} {
      \node[bclGeneratorStyle,rectStyle] (\name) at \coord {};
    }
    \foreach \name/\coord in {fd/\fd, td/\td, te/\te, tf/\tf, tg/\tg, P/\P, E/\E} {
      \node[faceStyle,circleStyle] (\name) at \coord {};
    }

    \foreach \from/\to in {E/va, E/vb, E/vc, E/vd, E/ve, E/vf, E/vg, E/vh, E/vi, E/vj, E/vk, E/vl, E/vm, 
        vd/ea, ve/ea, vd/eb, vg/eb, vj/ec, vk/ec,
        ec/fa,
        fb/ta, fb/tb, fc/tb, fc/tc,
        ta/P, tb/P, tc/P, td/P, te/P, tf/P, tg/P} {
      \draw[incidence] (\from) -- (\to);
    }
  
    % legend of face lattice
    \node[above] at (P.north) {$P$};
    \node[below] at (E.south) {$\emptyset$};
    \node[right] at (tg.east) {facets};
    \node[below=5pt] at (vm.east) {vertices};
    \node[above=12pt] at (vm.east) {edges};

    % legend of symbols
    \node[faceStyle,circleStyle] (legendFace) at (0.75,-2.3) {};
    \node[above] at (legendFace.north) {$F \notin \mathcal{F} \cup \mathcal{V}$};
    \node[bclVertexStyle,starStyle] (legendBclVertex) at (2.25,-2.3) {};
    \node[above] at (legendBclVertex.north) {$\mathcal{V}$};
    \node[bclFaceStyle,rectStyle] (legendBclFace) at (4.25,-2.3) {};
    \node[above] at (legendBclFace.north) {$\mathcal{F}$};
    \node[bclGeneratorStyle,rectStyle] (legendBclGenerator) at (5.0,-2.3) {};
    \node[right] at (legendBclGenerator.east) {\begin{minipage}{15mm}
        maximal elements in $\mathcal{F}$
      \end{minipage}};
  }{}
}


==> TikZ-extended-formulations-m-gon.tex <==
\piDeclareString{job}{}
\piDeclareBool{colors}{true}
\piDeclareBool{decorations}{true}

\piParse % Parses all given options

\piIfString{job}{config}{%
  % Preamble code
}{
  % Drawing code
  \draw[draw=none,clip,use as bounding box] (-5.7,-2) rectangle (5.5,5);

  \tikzset{
    node/.style={shape=circle,ball color=black,inner sep=0mm,minimum size=2mm,fill=white},
  }

  \foreach \id/\angle in {1/0, 2/22.5, 3/45, 4/67.5, 5/90, 6/112.5, 7/135, 8/157.5}{
    \coordinate (v\id) at ({0+4*cos(\angle)},{0+4*sin(\angle)});
  }
  
  \filldraw[black!10!white] (v1)--(v2)--(v3)--(v4)--(v5)--(v6)--(v7)--(v8)--(v1);
  \filldraw[black!20!white] (v1)--(v2)--(v3)--(v4)--(v1);
  \filldraw[very thick,black!90!white] (v1)--(v2)--(v1);

  \foreach \name/\angle/\style in {%
      {$H^{(2)}_{=}$}/{90-11.25}/{black!30!white},%
      {$H^{(1)}_{=}$}/{45-11.25}/{black!60!white},%
      {$H^{(0)}_{=}$}/{22.5-11.25}/{black!90!white}%
  }{
    \draw[\style] ({-2.7*cos(\angle)},{-2.7*sin(\angle)}) -- ({4.7*cos(\angle)},{4.7*sin(\angle)});
    \node[anchor=west] at ({4.7*cos(\angle)},{4.7*sin(\angle)}) {\name};
  }

  \foreach \id in {1,2,3,4,5,6,7,8}{
    \node[node] (node v\id) at (v\id) {};
    \node[below right] at (node v\id.south east) {$v_{\id}$};
  }
  
  \node[node] (origin) at (0,0) {};
  \node[below right] at (origin.south east) {$(0,0)$};
}


==> TikZ-extended-formulations-simple-acyclic-flows.tex <==
\piDeclareString{job}{}
\piDeclareBool{colors}{true}
\piDeclareBool{spindle}{false}
\piDeclareBool{decorations}{false}
\piDeclareBool{alternative path a}{false}
\piDeclareBool{alternative path b}{false}
\piDeclareBool{spindle path a}{false}
\piDeclareBool{spindle path b}{false}
\piDeclareBool{final paths}{false}

\piParse % Parses all given options

\piIfString{job}{config}{%
  % Preamble code
  \usetikzlibrary{arrows}
}{
  \piIfBool{colors}{
    \piIfBool{decorations}{
      \tikzset{
        >=stealth',
        node/.style={circle,draw=black,fill=white,inner sep=0mm,minimum size=1.5mm},
        edge/.style={semithick},
        edgeFixed/.style={orange!90!black,semithick,decorate,%
        decoration={coil,amplitude=1.7pt,segment length=1.9pt}},
        edgeGiven/.style={blue,edge},
        edgeAlternative/.style={green!70!black,edge,semithick,decorate,%
        decoration={zigzag,amplitude=1.5pt,segment length=3pt}},
        edgeSpindle1/.style={red,edge,densely dashed,very thick},
        edgeSpindle2/.style={purple!70!black,edge,dotted,very thick},
        edgePath/.style={edge,semithick,decorate,%
        decoration={snake,amplitude=1.5pt,segment length=3pt,pre length=1mm,post length=1.5mm}},
        spindle/.style={draw=black,fill=black!10!white,rounded corners=2mm},
      }
    }{
      \tikzset{
        >=stealth',
        node/.style={shape=circle,ball color=blue,fill=white,inner sep=0mm,minimum size=1.5mm},
        edge/.style={semithick,->},
        edgeFixed/.style={edge,orange!90!black},
        edgeGiven/.style={edge,blue},
        edgeAlternative/.style={edge,green!70!black},
        edgeSpindle1/.style={edge,red,ultra thick},
        edgeSpindle2/.style={edge,purple!70!black},
        edgePath/.style={edge,semithick,decorate,decoration={snake,amplitude=1.5pt,segment length=3pt,pre length=1mm,post length=1.5mm}},
        spindle/.style={draw=black,fill=yellow,fill opacity=0.3,rounded corners=2mm},
      }
    }
  }{
    \tikzset{
      node/.style={circle,draw=black,fill=white,inner sep=0mm,minimum size=1.5mm},
      edge/.style={semithick},
      edgeFixed/.style={semithick,decorate,decoration={coil,amplitude=1.7pt,segment length=1.9pt}},
      edgeGiven/.style={edge},
      edgeAlternative/.style={edge,semithick,decorate,decoration={zigzag,amplitude=1.5pt,segment length=3pt}},
      edgeSpindle1/.style={edge,densely dashed,ultra thick},
      edgeSpindle2/.style={edge,dotted},
      edgePath/.style={edge,semithick,decorate,decoration={snake,amplitude=1.5pt,segment length=3pt,pre length=1mm,post length=1.5mm}},
      spindle/.style={draw=black,fill=black!10!white,rounded corners=2mm},
    }
  }

  \def\commonDraw{
    % Setup coordinates
    \foreach \name/\x/\y in \Nodes
    {
      \coordinate (\name) at (\x,\y);
    }

    % Draw nodes
    \foreach \name/\x/\y in \Nodes
    {
      \node[node] (\name) at (\name) {};
    }

    % Draw arcs
    \foreach \u/\v/\style/\bend in \Arcs
    {
      \draw[\style] (\u) to[bend left=\bend] (\v);
    }

    % Draw node labels
    \foreach \name/\where/\distance/\label in \NodeLabels
    {
      \node[\where=\distance of \name] {\small{\label}};
    }
  }
  
  \piIfString{job}{cut-node}{
    \draw[clip,use as bounding box,draw=none] (-0.25,-0.5) rectangle +(4.5,1);

    \def\Nodes{
      s/0/0, t/4/0, b/2/0,
      a/0.45/0.3, c/0.3/-0.4, d/0.7/0.1, e/1.4/0.2,
      f/2.6/-0.1, g/3.1/-0.4, h/2.5/0.4}
    \def\Arcs{
      s/a/edge/0, s/c/edge/0, s/d/edge/0, 
      a/e/edge/10, 
      c/d/edge/0, c/b/edge/0,
      d/e/edge/-10,
      e/b/edge/0,
      b/h/edge/0, b/f/edge/0,
      f/g/edge/0,
      g/t/edge/0,
      h/g/edge/5, h/t/edge/0}
    \def\NodeLabels{
      s/below left/-1mm/{$s$},
      t/below right/-1mm/{$t$},
      b/below/0mm/{\footnotesize{cut-node}}}
  
    \commonDraw
  }{}

  \piIfString{job}{biclique layout}{
    \draw[clip,use as bounding box,draw=none] (-0.25,-1) rectangle +(10.5,2);

    \def\Nodes{s/0/0, t/10/0,
      Ba/1/0, Bb/3/0, Bc/4/0, Bd/5/0, Be/7/0, Bf/8/0}
    \def\Arcs{
      s/Ba/edgeFixed/0, Bb/Bc/edgeFixed/0, Bc/Bd/edgeFixed/0, Be/Bf/edgeFixed/0,
      Ba/Bb/edgePath/40, Ba/Bb/edgePath/0, Ba/Bb/edgePath/-40,
      Bd/Be/edgePath/45, Bd/Be/edgePath/15, Bd/Be/edgePath/-15, Bd/Be/edgePath/-45,
      Bf/t/edgePath/40, Bf/t/edgePath/0, Bf/t/edgePath/-40}
    \def\NodeLabels{
      s/below left/-1mm/{$s$},
      t/below right/-1mm/{$t$}}

    \piIfBool{spindle}{
      \foreach \x in {1,5,8}
      {
        \draw[spindle]
          (\x-0.3,0.2) -- (\x-0.3,-0.2) -- (\x+0.5,-0.65) -- (\x+0.8,-0.7) -- (\x+1.2,-0.7) -- (\x+1.5,-0.65) -- 
          (\x+2.15,-0.2) -- (\x+2.15,0.2) -- (\x+1.5,0.65) -- (\x+1.2,0.7) -- (\x+0.8,0.7) -- (\x+0.5,0.65) -- cycle;
      }
    }{}

    \commonDraw
  }{}

  \piIfString{job}{common neighbor}{
    \draw[clip,use as bounding box,draw=none] (-0.25,-3.2) rectangle +(10.5,4.9);

    \def\Nodes{s/0/0, t/10/0,
      x/3/0, y/6/0, sp/2/0, yp/7/0}
    \def\Arcs{
      s/sp/edgeGiven/-30, sp/x/edgeGiven/-30, x/y/edgeGiven/-30, y/yp/edgeGiven/-30, yp/t/edgeGiven/-30,
      sp/x/edgeFixed/0, y/yp/edgeFixed/0}
    \def\NodeLabels{
      s/below left/-1mm/{$s$},
      t/below right/-1mm/{$t$},
      x/below/0mm/{$x$},
      y/below/0mm/{$y$}}
    \def\Legend{
      0.5/-2.0/{$B$}/edgeFixed,
      1.75/-2.0/{$P$}/edgeGiven}

    \piIfBool{spindle}{
      \draw[spindle]
        (2.7,0.2) -- (2.7,-0.2) -- (3.8,-1.0) -- (4.3,-1.1) -- (4.7,-1.1) -- (5.2,-1.0) -- 
        (6.3,-0.2) -- (6.3,0.2) -- (5.2,1.0) -- (4.7,1.1) -- (4.3,1.1) -- (3.8,1.0) -- cycle;
      \node at (3.3,-0.9) {\small{$S$}};
    }{}

    \piIfBool{alternative path a}{
      \edef\Nodes{\Nodes}
      \edef\Arcs{\Arcs,
        s/sp/edgeAlternative/+30, sp/yp/edgeAlternative/+80, yp/t/edgeAlternative/+30}
      \edef\NodeLabels{\NodeLabels,
        sp/below/0mm/{$s'$},
        yp/below/0mm/{$t'$}}
      \edef\Legend{\Legend,
        3.0/-2.0/{$P'$}/edgeAlternative}

      \piIfBool{spindle path a}{
        \edef\Arcs{\Arcs,
          x/y/edgeSpindle1/-30}
        \edef\Legend{\Legend,
          1.125/-3.0/{$W$}/edgeSpindle1}
      }{}
      \piIfBool{spindle path b}{
        \edef\Arcs{\Arcs,
          x/y/edgeSpindle2/+30}
        \edef\Legend{\Legend,
          2.375/-3.0/{$W'$}/edgeSpindle2}
      }{}

      \piIfBool{final paths}{
        \edef\Nodes{\Nodes,
          f1s/6.0/-1.5, f1sp/6.67/-1.5, f1x/7.33/-1.5, f1y/8.67/-1.5, f1tp/9.33/-1.5, f1t/10/-1.5,
          f2s/6.0/-2.25, f2sp/6.67/-2.25, f2x/7.33/-2.25, f2y/8.67/-2.25, f2tp/9.33/-2.25, f2t/10/-2.25,
          f3s/6.0/-3.0, f3sp/6.67/-3.0, f3tp/9.33/-3.0, f3t/10/-3.0}
        \edef\Arcs{\Arcs,
          f1s/f1sp/edgeGiven/0, f1sp/f1x/edgeGiven/0, f1x/f1y/edgeSpindle1/0, f1y/f1tp/edgeGiven/0, f1tp/f1t/edgeGiven/0,
          f2s/f2sp/edgeGiven/0, f2sp/f2x/edgeGiven/0, f2x/f2y/edgeSpindle2/0, f2y/f2tp/edgeGiven/0, f2tp/f2t/edgeGiven/0,
          f3s/f3sp/edgeGiven/0, f3sp/f3tp/edgeAlternative/0, f3tp/f3t/edgeGiven/0}
        \edef\NodeLabels{\NodeLabels,
          f1s/above/-.5mm/{$s$}, f1sp/above/-.5mm/{$s'$}, f1x/above/-.5mm/{$x$},
          f1y/above/-.5mm/{$y$}, f1tp/above/-.5mm/{$t'$}, f1t/above/-.5mm/{$t$},
          f2s/above/-.5mm/{$s$}, f2sp/above/-.5mm/{$s'$}, f2x/above/-.5mm/{$x$},
          f2y/above/-.5mm/{$y$}, f2tp/above/-.5mm/{$t'$}, f2t/above/-.5mm/{$t$},
          f3s/above/-.5mm/{$s$}, f3sp/above/-.5mm/{$s'$}, f3tp/above/-.5mm/{$t'$}, f3t/above/-.5mm/{$t$}}
      }{}
    }{}

    \piIfBool{alternative path b}{
      \edef\Nodes{\Nodes,
        tp/5/0.95, tpp/5.4/0.6}
      \edef\Arcs{\Arcs,
        s/sp/edgeAlternative/+30, sp/tp/edgeAlternative/+70, tp/tpp/edgeAlternative/0, tpp/y/edgeAlternative/15, y/t/edgeAlternative/+30}
      \edef\NodeLabels{\NodeLabels,
        sp/below/0mm/{$s'$},
        tp/above/1mm/{$t'$},
        tpp/above right/0mm/{$t''$}}
      \edef\Legend{\Legend,
        3.0/-2.0/{$P'$}/edgeAlternative}

      \piIfBool{spindle path a}{
        \edef\Arcs{\Arcs,
          x/tp/edgeSpindle1/20}
        \edef\Legend{\Legend,
          1.125/-3.0/{$W$}/edgeSpindle1}
      }{}

      \piIfBool{spindle path b}{
        \edef\Arcs{\Arcs,
          x/tpp/edgeSpindle2/-20}
        \edef\Legend{\Legend,
          2.375/-3.0/{$W'$}/edgeSpindle2}
      }{}

      \piIfBool{final paths}{
        \edef\Nodes{\Nodes,
          f1s/6.0/-1.5, f1sp/6.67/-1.5, f1x/7.33/-1.5, f1tp/8/-1.5, f1tpp/8.67/-1.5, f1y/9.33/-1.5, f1t/10/-1.5,
          f2s/6.0/-2.25, f2sp/6.67/-2.25, f2x/7.33/-2.25,           f2tpp/8.67/-2.25, f2y/9.33/-2.25, f2t/10/-2.25,
          f3s/6.0/-3.0, f3sp/6.67/-3.0, f3tp/8/-3.0, f3tpp/8.67/-3.0, f3y/9.33/-3.0, f3t/10/-3.0}
        \edef\Arcs{\Arcs,
          f1s/f1sp/edgeGiven/0, f1sp/f1x/edgeGiven/0, f1x/f1tp/edgeSpindle1/0, f1tp/f1tpp/edgeAlternative/0, f1tpp/f1y/edgeAlternative/0, 
            f1y/f1t/edgeGiven/0,
          f2s/f2sp/edgeGiven/0, f2sp/f2x/edgeGiven/0, f2x/f2tpp/edgeSpindle2/0, f2tpp/f2y/edgeAlternative/0, f2y/f2t/edgeGiven/0,
          f3s/f3sp/edgeGiven/0, f3sp/f3tp/edgeAlternative/0, f3tp/f3tpp/edgeAlternative/0, f3tpp/f3y/edgeAlternative/0, f3y/f3t/edgeGiven/0}
        \edef\NodeLabels{\NodeLabels,
          f1s/above/-.5mm/{$s$}, f1sp/above/-.5mm/{$s'$}, f1x/above/-.5mm/{$x$}, f1tpp/above/-.5mm/{$t''$},
          f1y/above/-.5mm/{$y$}, f1tp/above/-.5mm/{$t'$}, f1t/above/-.5mm/{$t$},
          f2s/above/-.5mm/{$s$}, f2sp/above/-.5mm/{$s'$}, f2x/above/-.5mm/{$x$},
          f2y/above/-.5mm/{$y$}, f2tpp/above/-.5mm/{$t''$}, f2t/above/-.5mm/{$t$},
          f3s/above/-.5mm/{$s$}, f3sp/above/-.5mm/{$s'$}, f3tp/above/-.5mm/{$t'$}, f3tpp/above/-.5mm/{$t''$},
          f3y/above/-.5mm/{$y$}, f3t/above/-.5mm/{$t$}}
      }{}
    }{}

    \piIfBool{colors}{}{
      \node[anchor=west] at (-0.25,1.5) {\small{All arcs go from}};
      \node[anchor=west] at (-0.25,1.1) {\small{left to right.}};
    }

    \commonDraw
  }{}

  \piIfString{job}{cut-node}{
    \node[node,ball color=red] (b) at (b) {};
  }{}

  \piIfString{job}{biclique layout}{
    \node at (3.4,-0.4) {\small{$\textcolor{orange!90!black}{B}$}};
  }{}

  \piIfString{job}{common neighbor}{
    \foreach \x/\y/\name/\style in \Legend
    {
      \node[anchor=south] at (\x,\y) {\small{\name}};
      \draw[\style] (\x-0.4,\y) -- +(+0.8,0);
    }

    \piIfBool{final paths}{
      \foreach \i in {1,2,3}
      {
        \node[anchor=east] at (5.8,{-1.5 - (\i-1)*0.75}) {\small{$P_{\i} : $}};
      }
    }{}
  }{}

}

%\CommonNeighborfalse
%\ifCommonNeighbor
%  \draw[clip,use as bounding box,draw=none] (-4.1,-3.2) rectangle +(10.5,4.9);
%
% Drawing code
%
%  \tikzset{
%    vertex/.style={circle,draw=black,fill=white,inner sep=0mm,minimum size=2mm},
%    edge/.style={thick},
%  }

%	\ifDrawColors
%	  \tikzset{
%	    FixedStyle/.style={thick,orange},
%	    GivenPathStyle/.style={thick,blue},
%      AlternativePathStyle/.style={thick,green!70!black},
%	    SpindleOneStyle/.style={thick,red},
%	    SpindleTwoStyle/.style={thick,purple!70!black}
%    }
%	\else
%	  \tikzset{
%	    FixedStyle/.style={semithick,decorate,decoration={coil,amplitude=1.7pt,segment length=1.9pt}},
%	    GivenPathStyle/.style={thick},
%	    AlternativePathStyle/.style={semithick,decorate,decoration={zigzag,amplitude=1.5pt,segment length=3pt}},
%	    SpindleOneStyle/.style={thick,densely dashed},
%	    SpindleTwoStyle/.style={thick,dotted}
%    }
%	\fi
%
%\def\xscale{0.75}
%	
%\node[cloud, cloud puffs=21, draw, minimum width=26mm, minimum height=27mm] (Cloud) at (1.5*\xscale,-0.1) {};
%\node at (0.0*\xscale,-1.3) {\small{$S$}};
%
%\node[vertex] (s) at (-5*\xscale,0) {};
%\node[vertex] (v1) at (-4*\xscale,0) {};
%\node[vertex] (v2) at (-3*\xscale,0) {};
%\node[vertex] (sp) at (-2*\xscale,0) {};
%\node[vertex] (v3) at (-1*\xscale,0) {};
%\node[vertex] (x) at (0.1*\xscale,0) {};
%\node[vertex] (y) at (2.9*\xscale,0) {};
%\node[vertex] (v4) at (4*\xscale,0) {};
%\node[vertex] (v5) at (5*\xscale,0) {};
%\node[vertex] (v6) at (6*\xscale,0) {};
%\node[vertex] (v7) at (7*\xscale,0) {};
%\node[vertex] (t) at (8*\xscale,0) {};
%
%\node[vertex] (tp) at (1.5*\xscale,+1) {};
%\node[vertex] (S1) at (1*\xscale,-1) {};
%\node[vertex] (S2) at (2*\xscale,-1) {};
%\node[vertex] (S3) at (2*\xscale,+0.66) {};
%\node[vertex] (S4) at (2.5*\xscale,+0.33) {};
%\node[vertex] (S5) at (1.0*\xscale,+0.8) {};
%
%\node[vertex] (e1) at (-1.5*\xscale,+1) {};
%\node[vertex] (e2) at (-0.5*\xscale,+1.5) {};
%\node[vertex] (e3) at (6.5*\xscale,+0.6) {};
%
% node labels
%\node[below=3pt of s] {\small $s$};
%\node[below=3pt of sp] {\small $s'$};
%\node[below=2pt of x] {\small $x$};
%\node[below=2pt of y] {\small $y$};
%\node[below=3pt of t] {\small $t$};
%\node[above=3.5pt of tp] {\small $t'$};
	
% fixed edges
%\draw[edge,FixedStyle] (s) -- (v1) -- (v2) -- (sp) -- (v3) -- (x);
%\draw[edge,FixedStyle] (y) -- (v4);
%\draw[edge,FixedStyle] (v6) -- (v7);

% given path edges
%\draw[edge,GivenPathStyle] (s) 
%  ..controls(-4.8*\xscale,-0.2)and(-4.2*\xscale,-0.2).. (v1)
%  ..controls(-3.8*\xscale,-0.2)and(-3.2*\xscale,-0.2).. (v2)
%  ..controls(-2.8*\xscale,-0.2)and(-2.2*\xscale,-0.2).. (sp)
%  ..controls(-1.8*\xscale,-0.2)and(-1.2*\xscale,-0.2).. (v3)
%  ..controls(-0.8*\xscale,-0.2)and(-0.2*\xscale,-0.2).. (x);
%
%\draw[edge,GivenPathStyle] (x) 
%  -- (S1) 
%  ..controls(1.3*\xscale,-1.2)and(1.7*\xscale,-1.2).. (S2) 
%  -- (y);
%
%\draw[edge,GivenPathStyle] (y) 
%  ..controls(+3.2*\xscale,-0.2)and(+3.8*\xscale,-0.2).. (v4)
%  ..controls(+4.2*\xscale,-0.2)and(+4.8*\xscale,-0.2).. (v5)
%  ..controls(+5.2*\xscale,-0.2)and(+5.8*\xscale,-0.2).. (v6)
%  ..controls(+6.2*\xscale,-0.2)and(+6.8*\xscale,-0.2).. (v7)
%  ..controls(+7.2*\xscale,-0.2)and(+7.8*\xscale,-0.2).. (t);
%
% around path edges
%\draw[edge,AlternativePathStyle] (s)
%  ..controls(-4.8*\xscale,+0.4)and(-4.2*\xscale,+0.4).. (v1)
%  ..controls(-3.7*\xscale,-0.5)and(-2.3*\xscale,-0.5).. (sp)
%  -- (e1)
%  ..controls(-1*\xscale,1.4).. (e2)
%  -- (tp)
%  -- (S3)
%  -- (S4)
%  -- (y)
%  ..controls(3.3*\xscale,-0.5)and(4.7*\xscale,-0.5).. (v5)
%  ..controls(5.8*\xscale,+0.8).. (e3)
%  -- (v7)
%  ..controls(7.5*\xscale,+0.2).. (t);
%
%% W edges
%\draw[edge,SpindleOneStyle] (x)
%  ..controls(0.6*\xscale,+0.6).. (S5)
%  -- (tp)
%  ..controls(2.0*\xscale,1.1).. (S3)
%  ..controls(2.5*\xscale,0.7).. (S4)
%  ..controls(2.9*\xscale,0.4).. (y);
%
%% W' edges
%\draw[edge,SpindleTwoStyle] (x)
%  ..controls(1*\xscale,-0.3)and(1.3*\xscale,0.5).. (S3)
%  ..controls(2.1*\xscale,0.3).. (S4)
%  ..controls(2.45*\xscale,0.0).. (y);
%
%  % description
%  \node[anchor=west] at (-4.1,1.2) {\small{All arcs go from}};
%  \node[anchor=west] at (-4.1,0.8) {\small{left to right.}};
%
%  % edge legend
%  \node at (-3.5,-2.0) {$B$};
%  \draw[edge,FixedStyle] (-3.5-0.4,-2.3) -- (-3.5+0.4,-2.3);
%  
%  \node at (-2.0,-2.0) {$P$};
%  \draw[edge,GivenPathStyle] (-2.0-0.4,-2.3) -- (-2.0+0.4,-2.3);
%
%  \node at (-0.5,-2.0) {$P'$};
%  \draw[edge,AlternativePathStyle] (-0.5-0.4,-2.3) -- (-0.5+0.4,-2.3);
%
%  \def\xshift{0.7}
%  \def\yshift{0.2}
%  \node at (-4+\xshift,-3.0+\yshift) {$W$};
%  \draw[edge,SpindleOneStyle] (-4.0-0.4+\xshift,-3.3+\yshift) -- (-4.0+0.4+\xshift,-3.3+\yshift);
%  
%  \node at (-1-\xshift,-3.0+\yshift) {$W'$};
%  \draw[edge,SpindleTwoStyle] (-1.0-0.4-\xshift,-3.3+\yshift) -- (-1.0+0.4-\xshift,-3.3+\yshift);
%
%  % path legend
%  \node (P1) at (-0.8+2.3,-2.0) {$P_1:$};
%  \node (P1 s) at (-0.8+3.0,-2.0) {$s$\textcolor{white}{'}};
%  \node (P1 sp) at (-0.8+4.0,-2.0) {$s'$};
%  \node (P1 x) at (-0.8+5.0,-2.0) {$x$\textcolor{white}{'}};
%  \node (P1 y) at (-0.8+6.0,-2.0) {$y$\textcolor{white}{'}};
%  \node (P1 t) at (-0.8+7.0,-2.0) {$t$\textcolor{white}{'}};
%  \draw[edge,GivenPathStyle] (P1 s) -- (P1 sp);
%  \draw[edge,GivenPathStyle] (P1 sp) -- (P1 x);
%  \draw[edge,SpindleOneStyle] (P1 x) -- (P1 y);
%  \draw[edge,GivenPathStyle] (P1 y) -- (P1 t);
%  
%  \node (P2) at (-0.8+2.3,-2.5) {$P_2:$};
%  \node (P2 s) at (-0.8+3.0,-2.5) {$s$\textcolor{white}{'}};
%  \node (P2 sp) at (-0.8+4.0,-2.5) {$s'$};
%  \node (P2 x) at (-0.8+5.0,-2.5) {$x$\textcolor{white}{'}};
%  \node (P2 y) at (-0.8+6.0,-2.5) {$y$\textcolor{white}{'}};
%  \node (P2 t) at (-0.8+7.0,-2.5) {$t$\textcolor{white}{'}};
%  \draw[edge,GivenPathStyle] (P2 s) -- (P2 sp);
%  \draw[edge,GivenPathStyle] (P2 sp) -- (P2 x);
%  \draw[edge,SpindleTwoStyle] (P2 x) -- (P2 y);
%  \draw[edge,GivenPathStyle] (P2 y) -- (P2 t);
%  
%  \node (P3) at (-0.8+2.3,-3.0) {$P_3:$};
%  \node (P3 s) at (-0.8+3.0,-3.0) {$s$\textcolor{white}{'}};
%  \node (P3 sp) at (-0.8+4.0,-3.0) {$s'$};
%  \node (P3 tp) at (-0.8+5.0,-3.0) {$t'$};
%  \node (P3 y) at (-0.8+6.0,-3.0) {$y$\textcolor{white}{'}};
%  \node (P3 t) at (-0.8+7.0,-3.0) {$t$\textcolor{white}{'}};
%  \draw[edge,GivenPathStyle] (P3 s) -- (P3 sp);
%  \draw[edge,AlternativePathStyle] (P3 sp) -- (P3 tp);
%  \draw[edge,SpindleOneStyle] (P3 tp) -- (P3 y);
%  \draw[edge,GivenPathStyle] (P3 y) -- (P3 t);


==> TikZ-extended-formulations-simple-extensions.tex <==
\piDeclareString{job}{}
\piDeclareBool{colors}{true}
\piDeclareBool{decorations}{true}

\piParse % Parses all given options

\piIfString{job}{config}{%
  % Preamble code
  \usetikzlibrary{positioning}
}{
  \piIfString{job}{example-polytope}{
    \tikzset{
      Qvertex/.style={circle,draw=black,fill=black,minimum size=1mm,inner sep=0.3mm},
      Pvertex/.style={circle,draw=black,fill=black,minimum size=1mm,inner sep=0.3mm}
    }

    \piIfBool{colors}{
      \fill[fill=blue!80!white] (5.7,4.8) -- (5.3,4.5) -- (3.9,4.3) -- cycle;
      \fill[fill=blue!80!white] (4.9,3.1) -- (5.3,4.5) -- (6.7,3.6) -- cycle;
    }{}

    \node[Qvertex] (Q1) at (5.7,4.8) {};
    \node[Qvertex] (Q2) at (8.4,3.0) {};
    \node[Qvertex] (Q3) at (6.7,3.6) {};
    \node[Qvertex] (Q4) at (5.3,4.5) {};
    \node[Qvertex] (Q5) at (3.9,4.3) {}; 
    \node[Qvertex] (Q6) at (2.0,1.25) {};
    \node[Qvertex] (Q7) at (4.9,3.1) {};

    \node[above=0pt of Q1] {$m_1$};
    \node[below=0pt of Q2] {$m_2$};
    \node[below=0pt of Q3] {$m_3$};
    \node[right=0pt of Q4] {$m_4$};
    \node[left=0pt of Q5] {$m_5$};
    \node[left=0pt of Q6] {$m_6$};
    \node[below=0pt of Q7] {$m_7$};

    \draw (Q1) -- (Q2);
    \draw (Q1) -- (Q4);
    \draw (Q1) -- (Q5);
    \draw (Q2) -- (Q3);
    \draw (Q2) -- (Q6);
    \draw (Q3) -- (Q4);
    \draw (Q3) -- (Q7);
    \draw (Q4) -- (Q5);
    \draw (Q4) -- (Q7);
    \draw (Q5) -- (Q6);
    \draw (Q6) -- (Q7);

    \node[Pvertex] (P1) at (5.7,4.8 - 3.5) {}; %
    \node[Pvertex] (P2) at (8.4,3.0 - 3.5 + 1.8) {};
    \node[Pvertex] (P3) at (6.7,3.6 - 3.5) {}; %
    \node[Pvertex] (P4) at (5.3,4.5 - 3.5 - 0.55) {};
    \node[Pvertex] (P5) at (3.9,4.3 - 3.5) {}; % 
    \node[Pvertex] (P6) at (2.0,1.25- 3.5 + 1.8) {};
    \node[Pvertex] (P7) at (4.9,3.1 - 3.5) {}; %

    \draw (P1) -- (P2);
    \draw[dashed] (P1) -- (P4);
    \draw (P1) -- (P5);
    \draw (P2) -- (P3);
    \draw[dashed] (P2) -- (P6);
    \draw[dashed] (P3) -- (P4);
    \draw (P3) -- (P7);
    \draw[dashed] (P4) -- (P5);
    \draw[dashed] (P4) -- (P7);
    \draw (P5) -- (P6);
    \draw (P6) -- (P7);

    \draw[very thick,->] (10,3.0) -- node[right=1pt] {$\pi$} (10,1.5);

    \node at (2.5,3) {$Q$};
    \node at (8,0) {$P = \pi(Q)$};

  }{}
}


==> TikZ-extended-formulations-simple-hypersimplex.tex <==
\piDeclareString{job}{}
\piDeclareBool{colors}{true}
\piDeclareBool{decorations}{true}
\piDeclareBool{shift}{false}

\piParse % Parses all given options

\piIfString{job}{config}{%
  % Preamble code
}{
  \piIfString{job}{hypersimplex}{

    \piIfBool{colors}{
      \def\redzero{\textcolor{red}{0}}
      \def\bluezero{\textcolor{blue}{0}}
      \def\greenzero{\textcolor{green!70!black}{0}}
      \def\redone{\textcolor{red}{1}}
      \def\blueone{\textcolor{blue}{1}}
      \def\greenone{\textcolor{green!70!black}{1}}
    }{
      \def\redzero{0}
      \def\bluezero{0}
      \def\greenzero{0}
      \def\redone{1}
      \def\blueone{1}
      \def\greenone{1}
    }

    % table
    \foreach \x in {2, 4} {
      \draw (\x,0.5) -- (\x,-3.5);
    }

    \node[anchor=south] at (1,0) {$L$};
    \node[anchor=south] at (3,0) {$U$};
    \node[anchor=south] at (5,0) {$R$};
  
    \draw (0,0) -- (6.5,0);

    \node at (1,-0.5) {$1,1,\ldots,1,1$};
    \node at (0.5,-1.25) {$\vdots$};
    \node at (1.5,-1.25) {$\vdots$};
    \node at (1,-2.0) {$1,1,\ldots,1,1$};
    \node at (3,-0.5) {$0,0,\ldots,0,0$};
    \node at (2.5,-1.25) {$\vdots$};
    \node at (3.5,-1.25) {$\vdots$};
    \node at (3,-2.0) {$0,0,\ldots,0,0$};

    \node at (5.25,-0.5) {$\ldots,\redzero,\ldots,\blueone,\ldots$};
    \node at (5.25,-2.0) {$\ldots,\redone,\ldots,\bluezero,\ldots$};

    \draw (0,-2.5) -- (6.5,-2.5);

    \node at (1,-2.75) {$\greenzero,1,\ldots,1,1$};
    \node at (3,-2.75) {$0,0,\ldots,0,0$};
    \node at (5.25,-2.75) {$\ldots,\redone,\ldots,\blueone,\ldots$};
  
    \draw (0,-3.0) -- (6.5,-3.0);
  
    \node at (1,-3.25) {$1,1,\ldots,1,1$};
    \node at (3,-3.25) {$\greenone,0,\ldots,0,0$};
    \node at (5.25,-3.25) {$\ldots,\redzero,\ldots,\bluezero,\ldots$};

    % brace
    \draw[decorate,decoration={brace,amplitude=10pt},xshift=7pt,yshift=0mm]
      (6.75,0) -- (6.75,-2.5) node [black,midway,xshift=7mm] {$\mathcal{V}$};

    % labels

    \node at (-0.5,-0.5) {$u = $};
    \node at (-0.5,-2.0) {$w = $};

    \piIfBool{colors}{
      \piIfBool{shift}{
        \node at (4.8+0.07,-4) {\textcolor{red}{$i$}};
        \draw[red,->] (4.8+0.07,-3.8) -- (4.8+0.07,-3.5);
        \node at (5.7-0.03,-4) {\textcolor{blue}{$j$}};
        \draw[blue,->] (5.7-0.03,-3.8) -- (5.7-0.03,-3.5);
      }{
        \node at (4.8+0.02,-4) {\textcolor{red}{$i$}};
        \draw[red,->] (4.8+0.02,-3.8) -- (4.8+0.02,-3.5);  
        \node at (5.7+0.05,-4) {\textcolor{blue}{$j$}};
        \draw[blue,->] (5.7+0.05,-3.8) -- (5.7+0.05,-3.5);
      }
      \node at (8,-3) {$\textcolor{green!70!black}{v} \notin \mathcal{V}$};
      \draw[green!70!black,->] (7.5,-2.9) -- (7.0,-2.75);  
      \draw[green!70!black,->] (7.5,-3.1) -- (7.0,-3.25);  
    }{
      \piIfBool{shift}{
        \node at (4.8+0.07,-4) {$i$};
        \draw[->] (4.8+0.07,-3.8) -- (4.8+0.07,-3.5);
        \node at (5.7-0.03,-4) {$j$};
        \draw[->] (5.7-0.03,-3.8) -- (5.7-0.03,-3.5);
      }{
        \node at (4.8+0.02,-4) {$i$};
        \draw[->] (4.8+0.02,-3.8) -- (4.8+0.02,-3.5);  
        \node at (5.7+0.05,-4) {$j$};
        \draw[->] (5.7+0.05,-3.8) -- (5.7+0.05,-3.5);
      }
      \node at (8,-3) {$v \notin \mathcal{V}$};
      \draw[->] (7.5,-2.9) -- (7.0,-2.75);  
      \draw[->] (7.5,-3.1) -- (7.0,-3.25);  
    }
 
   \piIfBool{shift}{
    \node at (1.25+0.1,-4.0) {$s$};
    \draw[->] (1.0+0.1,-4.0) ..controls(0.2+0.1,-4.0).. (0.2+0.1,-3.5);  
    \draw[->] (1.5+0.1,-4.0) ..controls(2.2+0.1,-4.0).. (2.2+0.1,-3.5);
   }{ 
    \node at (1.25,-4.0) {$s$};
    \draw[->] (1.0,-4.0) ..controls(0.2,-4.0).. (0.2,-3.5);  
    \draw[->] (1.5,-4.0) ..controls(2.2,-4.0).. (2.2,-3.5);
   }
  }{}
}


==> TikZ-extended-formulations-simple-matchings.tex <==
\piDeclareBool{argumentation}{false}
\piDeclareBool{set}{false}
\piDeclareBool{operation}{false}
\piDeclareBool{violated}{false}

\piParse

% Drawing code

\piIfBool{argumentation}{
  \draw[clip,use as bounding box,draw=none] (-4.25,-1.1) rectangle +(8.5,2.2);
  
  \tikzset{
    node/.style={shape=circle,ball color=blue,inner sep=0mm,minimum size=2mm,fill=white},
    edge/.style={black!80!white,very thick},
    set/.style={draw=black,fill=red!80!white,rounded corners=1.5mm},
  }

  \piIfBool{set}{
    \draw[set] (-0.3-2.5,+0.6) -- (+0-2.5,+0.75) -- (+0.3-2.5,+0.6) -- (+0.3-2.5,-0.6) -- (+0-2.5,-0.75) -- (-0.3-2.5,-0.6) -- cycle;
    \draw[set] (-0.3+0.5,+0.6) -- (+0+0.5,+0.75) -- (+0.3+0.5,+0.6) -- (+0.3+0.5,-0.6) -- (+0+0.5,-0.75) -- (-0.3+0.5,-0.6) -- cycle;
    \piIfBool{operation}{
      \draw[set] (-0.3+3.5,+0.6) -- (+0+3.5,+0.75) -- (+0.3+3.5,+0.6) -- (+0.3+3.5,-0.6) -- (+0+3.5,-0.7) -- (-1.0+3.5,-0.7)
        -- (-1.3+3.5,-0.5) -- cycle;
    }{
      \draw[set] (-0.3+3.5,+0.6) -- (+0+3.5,+0.75) -- (+0.3+3.5,+0.6) -- (+0.3+3.5,-0.6) -- (+0+3.5,-0.75) -- (-0.3+3.5,-0.6) -- cycle;
    }
  }{}
  
  % left
  
  \node[node] (left M1) at (-3.5,+0.5) {};
  \node[node] (left M2) at (-2.5,+0.5) {};
  \node[node] (left M3) at (-2.5,-0.5) {};
  \draw[edge] (left M1) -- (left M2);
  
  \node[above=0 of left M1] {\footnotesize{$\chi(M_1)$}};
  \node[above=0 of left M2] {\footnotesize{$\chi(M_2)$}};
  \node[below=0 of left M3] {\footnotesize{$\chi(M_3)$}};
  
  % arrow
  
  \node at (-1.5,0) {\LARGE{$\Rightarrow$}};
  
  % middle
  
  \node[node] (middle M1) at (-0.5,+0.5) {};
  \node[node] (middle M2) at (+0.5,+0.5) {};
  \node[node] (middle M3) at (+0.5,-0.5) {};
  \draw[edge] (middle M1) -- (middle M2) -- (middle M3) -- (middle M1);
  
  \node[above=0 of middle M1] {\footnotesize{$\chi(M_1)$}};
  \node[above=0 of middle M2] {\footnotesize{$\chi(M_2)$}};
  \node[below=0 of middle M3] {\footnotesize{$\chi(M_3)$}};
  
  \node at (+1.5,0) {\large{or}};
  
  % right
  
  \node[node] (right M1) at (+2.5,+0.5) {};
  \node[node] (right M2) at (+3.5,+0.5) {};
  \node[node] (right M3) at (+3.5,-0.5) {};
  \node[node] (right Mprime) at (+2.5,-0.5) {};
  \draw[edge] (right M1) -- (right M2) -- (right Mprime) -- (right M1);
  \draw[edge] (right Mprime) -- (right M3);
  
  \node[above=0 of right M1] {\footnotesize{$\chi(M_1)$}};
  \node[above=0 of right M2] {\footnotesize{$\chi(M_2)$}};
  \node[below=0 of right M3] {\footnotesize{$\chi(M_3)$}};
  \node[below=0 of right Mprime] (right Mprime label) {\footnotesize{$\chi(\textcolor{cyan}{M'})$}};
  
  \node[left=-2mm of right Mprime label] {\footnotesize{$\textcolor{cyan}{\exists}$}};

  \piIfBool{violated}{
    \draw[edge,cyan,decorate,decoration={zigzag,segment length=2mm, amplitude=0.8mm}] (middle M2) -- (middle M1) -- (middle M3);
    \piIfBool{operation}{
      \draw[edge,cyan,decorate,decoration={zigzag,segment length=2mm, amplitude=0.8mm}] (right M2) -- (right M1) -- (right Mprime);
    }{
      \draw[edge,cyan,decorate,decoration={zigzag,segment length=2mm, amplitude=0.8mm}] (right M2) -- (right Mprime) -- (right M3);
    }
  }{}
}{}


==> TikZ-extended-formulations-simple-spanning-tree.tex <==
\piDeclareString{job}{}
\piDeclareBool{colors}{true}
\piDeclareBool{decorations}{true}

\piParse % Parses all given options

\piIfString{job}{config}{%
  % Preamble code
  \usetikzlibrary{shapes.symbols}
  \usetikzlibrary{positioning}
}{
  \piIfString{job}{common-neighbors}{

    \tikzset{
	    vertex/.style={circle,draw=black,minimum size=2mm},
	    edge/.style={thick},
	  }

    \piIfBool{colors}{
      \tikzset{
	      redStyle/.style={thick,red},
	      greenStyle/.style={thick,green!70!black},
	      blueStyle/.style={thick,blue},
	      orangeStyle/.style={thick,orange},
	      purpleStyle/.style={thick,purple!70!black}
	    }
    }{
	    \tikzset{
	      redStyle/.style={thick},
	      greenStyle/.style={thick},
	      blueStyle/.style={thick},
	      orangeStyle/.style={thick},
	      purpleStyle/.style={thick}
	    }
    }
	
	  % vertex clouds
	  \node[cloud, cloud puffs=11, draw, minimum width=2cm, minimum height=2cm] (X1) at (-1.5,1.0) {};
	  \node at (-1.5,1.0) {\small{$X'$}};
	  \node[cloud, cloud puffs=14, draw, minimum width=3cm, minimum height=2cm] (X2) at (2,1.0) {};
	  \node at (2,1.0) {\small{$X''$}};
	  \node[cloud, cloud puffs=20, draw, minimum width=5cm, minimum height=3cm] (Y) at (0.5,-2.0) {};
	  \node at (0.5,-2.0) {\small{$Y$}};
	
	  % edges
	  \draw[edge,redStyle]    (X2) .. controls (1.3,0.3) and (0.8,-0.6) ..    node[left,midway,redStyle] {$e$} (Y);
	  \draw[edge,greenStyle]  (X2) .. controls (2.5,0.1) and (2.8,-0.6) ..    node[left,midway,greenStyle] {$f$} (Y);
	  \draw[edge,blueStyle]   (X1) .. controls (-0.2,1.8) and (0.3,1.8) ..    node[above,midway,blueStyle] {$g$} (X2);
	  \draw[edge,orangeStyle] (X1) .. controls (-0.2,0.5) and (0.3,0.5) ..    node[above,midway,orangeStyle] {$h$} (X2);
	  \draw[edge,purpleStyle] (X1) .. controls (-1.5,-0.2) and (-1.3,-0.6) .. node[left,midway,purpleStyle] {$j$} (Y);
  }{}

  \piIfString{job}{simple-bicliques}{
    \tikzset{
	    vertex/.style={circle,draw=black},
	    edge/.style={thick},
  	}
	  \piIfBool{colors}{
      \piIfBool{decorations}{
        \tikzset{
          redStyle/.style={red,semithick,decorate,%
          decoration={zigzag,amplitude=1.5pt,segment length=3pt}},
          blueStyle/.style={blue,semithick,decorate,%
          decoration={coil,amplitude=1.9pt,segment length=2pt}},
          redDashedStyle/.style={redStyle,dashdotted},
          blueDashedStyle/.style={blueStyle,dashdotted},
        }
      }{
	      \tikzset{
  	      redStyle/.style={thick,red},
	        blueStyle/.style={thick,blue},
	        redDashedStyle/.style={redStyle,dashed},
	        blueDashedStyle/.style={blueStyle,dashed},
        }
      }
    }{
	    \tikzset{
	      redStyle/.style={semithick,decorate,decoration={zigzag,amplitude=1.5pt,segment length=3pt}},
	      blueStyle/.style={semithick,decorate,decoration={coil,amplitude=1.9pt,segment length=2pt}},
	      redDashedStyle/.style={redStyle},
	      blueDashedStyle/.style={blueStyle},
	    }
	  }

	  % cloud for U
	  \node[gray!80!black,cloud, cloud puffs=20, draw, minimum width=12mm, minimum height=12mm] (U) at (-3,1.2) {};
	  \node[above left=0pt of U] {\textcolor{gray!80!black}{\small $U$}};

	  % vertices
	  \node[vertex] (s) at (-6,0) {};
	  \node[vertex] (w0) at (-5,0) {};
	  \node[vertex] (x) at (-4,0) {};
	  \node[vertex] (y) at (-3,1) {};
	  \node[vertex] (z) at (-2,0) {};
	  \node[vertex] (wk) at (-1,0) {};
	  \node[vertex] (t) at (0,0) {};

  	\node[vertex] (v1) at (1,0) {};
	  \node[vertex] (v2) at (1,-1) {};
	  \node[vertex] (v3) at (1,+1) {};
	  \node[vertex] (v4) at (1,-2) {};
	  \node[vertex] (v5) at (1,+2) {};
	  \node[vertex] (v6) at (1,-3) {};
	  \node[vertex] (v7) at (1,+3) {};

  	\node[above=0pt of s] {\small $s$};
	  \node[above=0pt of w0] {\small $w_1$};
  	\node[above=0pt of x] {\small $x$};
	  \node[above=0pt of y] {\small $y$};
  	\node[above=0pt of z] {\small $z$};
	  \node[above=0pt of wk] {\small $w_k$};
	  \node[above left=0pt of t] {\small $t$};

  	\node[right=0pt of v7] {\small $v_1$};
	  \node[right=0pt of v5] {\small $v_2$};
	  \node[right=2pt of v3]{\small $\vdots$};

  	% edges
	  \draw[edge,blueStyle] (s) ..controls(-5.5,0.15).. (w0);
	  \draw[edge,redStyle]  (s) ..controls(-5.5,-0.15).. (w0);

  	\draw[edge,blueDashedStyle] (w0) ..controls(-4.5,0.15).. (x);
	  \draw[edge,redDashedStyle]  (w0) ..controls(-4.5,-0.15).. (x);

  	\draw[edge,blueStyle] (x) ..controls(-3.5,0.15+0.5).. node[above left,midway,blueStyle] {$a$} (y);

  	\draw[edge,redStyle]  (x) ..controls(-3.5,-0.4)and(-2.5,-0.4).. node[below,midway,redStyle] {$b$} (z);

  	\draw[edge,blueStyle] (y) ..controls(-2.5,0.15+0.5).. node[above right,midway,black] {$c$} (z);
	  \draw[edge,redStyle]  (y) ..controls(-2.6,-0.15+0.4).. (z);

  	\draw[edge,blueDashedStyle] (z) ..controls(-1.5,0.15).. (wk);
	  \draw[edge,redDashedStyle]  (z) ..controls(-1.5,-0.15).. (wk);

  	\draw[edge,blueStyle] (wk) ..controls(-0.5,0.15).. (t);
	  \draw[edge,redStyle]  (wk) ..controls(-0.5,-0.15).. (t);

  	\draw[edge,blueStyle] (t) ..controls(+0.5,0.15).. (v1);
	  \draw[edge,redStyle]  (t) ..controls(+0.5,-0.15).. (v1);

  	\draw[edge,blueStyle] (t) ..controls(+0.5,-0.5+0.15).. (v2);
	  \draw[edge,redStyle]  (t) ..controls(+0.5,-0.5-0.15).. (v2);

  	\draw[edge,blueStyle] (t) ..controls(+0.5,+0.5+0.15).. (v3);
	  \draw[edge,redStyle]  (t) ..controls(+0.5,+0.5-0.15).. (v3);

  	\draw[edge,blueStyle] (t) ..controls(+0.5,-1.4+0.25).. (v4);
	  \draw[edge,redStyle]  (t) ..controls(+0.5,-1.4-0.15).. (v4);

  	\draw[edge,blueStyle] (t) ..controls(+0.5,+1.4+0.15).. (v5);
	  \draw[edge,redStyle]  (t) ..controls(+0.5,+1.4-0.25).. (v5);

  	\draw[edge,blueStyle] (t) ..controls(+0.1,-2.2+0.15).. (v6);
	  \draw[edge,redStyle]  (t) ..controls(-0.1,-2.2-0.35).. (v6);

  	\draw[edge,blueStyle] (t) ..controls(-0.1,+2.2+0.35).. (v7);
	  \draw[edge,redStyle]  (t) ..controls(+0.1,+2.2-0.15).. (v7);

  	% brace
	  \draw[decorate,decoration={brace,amplitude=10pt},xshift=0pt,yshift=-7mm]
	    (-0.9,0) -- (-5.1,0) node [black,midway,yshift=-7mm] {$W$};

  	% legend
	  \def\x{-5.2}
	  \def\y{-2.9}
	  \def\horzDist{0.5}
	  \def\horzStep{1.5}

  	\node[anchor=south] at (\x+0*\horzStep,\y) {\small $T(W)$};
	  \draw[blueStyle] (\x+0*\horzStep-\horzDist,\y) -- (\x+0*\horzStep+\horzDist,\y);

  	\node[anchor=south] at (\x+1*\horzStep,\y) {\small $T'$};
	  \draw[redStyle] (\x+1*\horzStep-\horzDist,\y) -- (\x+1*\horzStep+\horzDist,\y);
  }{}
}


==> TikZ-matchings-common-neighbor.tex <==
\piDeclareString{job}{}
\piDeclareBool{colors}{true}
\piDeclareBool{decorations}{true}

\piParse % Parses all given options

\piIfString{job}{config}{%
  % Preamble code
}{
  % Drawing code
  \tikzset{
    vertex/.style={circle,draw=black,minimum size=2mm},
    edge/.style={},
  }

  \piIfBool{colors}{
    \piIfBool{decorations}{
      \tikzset{
        redStyle/.style={red,semithick,decorate,decoration={zigzag,amplitude=1.5pt,segment length=3pt}},
        greenStyle/.style={green!70!black,semithick,decorate,decoration={coil,amplitude=1.9pt,segment length=2pt}},
        blueStyle/.style={blue,thick,dashed},
        orangeStyle/.style={orange,very thick,dotted}
      }
    }{
      \tikzset{
        redStyle/.style={thick,red},
        greenStyle/.style={thick,green!70!black},
        blueStyle/.style={thick,blue},
        orangeStyle/.style={thick,orange}
      }
    }
  }{
    \tikzset{
      redStyle/.style={semithick,decorate,decoration={zigzag,amplitude=1.5pt,segment length=3pt}},
      greenStyle/.style={semithick,decorate,decoration={coil,amplitude=1.9pt,segment length=2pt}},
      blueStyle/.style={thick,dashed},
      orangeStyle/.style={thick,dotted}
    }
  }

  \piIfString{job}{legend existence}{
    \def\vertDist{0.1}
    \def\horzDist{0.5}
    \def\horzStep{1.5}
  
    \node[anchor=south] at (0*\horzStep,0) {\small $M_1$};
    \draw[redStyle] (0*\horzStep-\horzDist,-\vertDist) -- (0*\horzStep+\horzDist,-\vertDist);
  
    \node[anchor=south] at (1*\horzStep,0) {\small $M_2$};
    \draw[greenStyle] (1*\horzStep-\horzDist,-\vertDist) -- (1*\horzStep+\horzDist,-\vertDist);
  
    \node[anchor=south] at (2*\horzStep,0) {\small $M_3$};
    \draw[orangeStyle] (2*\horzStep-\horzDist,-\vertDist) -- (2*\horzStep+\horzDist,-\vertDist);
  
    \node[anchor=south] at (3*\horzStep,0) {\small $M'$};
    \draw[blueStyle] (3*\horzStep-\horzDist,-\vertDist) -- (3*\horzStep+\horzDist,-\vertDist);
  }{}
  
  \piIfString{job}{legend switchings}{
    \def\vertDist{0.1}
    \def\horzDist{0.5}
    \def\horzStep{1.5}
  
    \node[anchor=south] at (0*\horzStep,0) {\small $M_j$};
    \draw[redStyle] (0*\horzStep-\horzDist,-\vertDist) -- (0*\horzStep+\horzDist,-\vertDist);
  
    \node[anchor=south] at (1*\horzStep,0) {\small $M_k$};
    \draw[greenStyle] (1*\horzStep-\horzDist,-\vertDist) -- (1*\horzStep+\horzDist,-\vertDist);
  
    \node[anchor=south] at (2*\horzStep,0) {\small $M_3$};
    \draw[orangeStyle] (2*\horzStep-\horzDist,-\vertDist) -- (2*\horzStep+\horzDist,-\vertDist);
  
    \node[anchor=south] at (3*\horzStep,0) {\small $M'$, $M^*$};
    \draw[blueStyle] (3*\horzStep-\horzDist,-\vertDist) -- (3*\horzStep+\horzDist,-\vertDist);
  }{}

  \piIfString{job}{adjacent-cycle}{
    % C12

    \foreach \i in {0,1,2,3,4,5,6,7,8,9,10,11}
    {
      \def\arc{-\i*360/12+90}
      \def\radius{1.4}
      \def\x{0.5}
      \def\y{0.0}
      \node[vertex,label=\arc:{\small $v_{\i}$}] (C12 \i) 
        at ({\radius*cos(\arc)+\x},{\radius*sin(\arc)+\y}) {};
    }

    \draw[edge,redStyle]   (C12 0) -- (C12 1);
    \draw[edge,greenStyle] (C12 1) -- (C12 2);
    \draw[edge,redStyle]   (C12 2) -- (C12 3);
    \draw[edge,greenStyle] (C12 3) -- (C12 4);
    \draw[edge,redStyle]   (C12 4) -- (C12 5);
    \draw[edge,greenStyle] (C12 5) -- (C12 6);
    \draw[edge,redStyle]   (C12 6) -- (C12 7);
    \draw[edge,greenStyle] (C12 7) -- (C12 8);
    \draw[edge,redStyle]   (C12 8) -- (C12 9);
    \draw[edge,greenStyle] (C12 9) -- (C12 10);
    \draw[edge,redStyle]   (C12 10) -- (C12 11);
    \draw[edge,greenStyle] (C12 11) -- (C12 0);

    \draw[edge,blueStyle]   (C12 0) ..controls({0.5+0.9*cos(+15.5)},{0.9*sin(+15.5)}).. (C12 2);
    \draw[edge,blueStyle]   (C12 3) ..controls({0.5+0.9*cos(+15.5)},{0.9*sin(+15.5)}).. (C12 5);
    \draw[edge,blueStyle]   (C12 4) -- (C12 7);
    \draw[edge,blueStyle]   (C12 6) -- (C12 9);
    \draw[edge,blueStyle]   (C12 8) -- (C12 11);
    \draw[edge,blueStyle]   (C12 10) -- (C12 1);

    % C10

    \foreach \i in {0,1,2,3,4,5,6,7,8,9}
    {
      \def\arc{-\i*360/10+90}
      \def\radius{1.25}
      \def\x{-3.8}
      \def\y{0.0}
      \node[vertex,label=\arc:{\small $v_{\i}$}] (C10 \i) at ({\radius*cos(\arc)+\x},{\radius*sin(\arc)+\y}) {};
    }

    \draw[edge,redStyle]   (C10 0) -- (C10 1);
    \draw[edge,greenStyle] (C10 1) -- (C10 2);
    \draw[edge,redStyle]   (C10 2) -- (C10 3);
    \draw[edge,greenStyle] (C10 3) -- (C10 4);
    \draw[edge,redStyle]   (C10 4) -- (C10 5);
    \draw[edge,greenStyle] (C10 5) -- (C10 6);
    \draw[edge,redStyle]   (C10 6) -- (C10 7);
    \draw[edge,greenStyle] (C10 7) -- (C10 8);
    \draw[edge,redStyle]   (C10 8) -- (C10 9);
    \draw[edge,greenStyle] (C10 9) -- (C10 0);

    \draw[edge,blueStyle] (C10 0) -- (C10 3);
    \draw[edge,blueStyle] (C10 2) -- (C10 5);
    \draw[edge,blueStyle] (C10 4) -- (C10 7);
    \draw[edge,blueStyle] (C10 6) -- (C10 9);
    \draw[edge,blueStyle] (C10 8) -- (C10 1);
  }{}

  \piIfString{job}{connect-outer-cycles}{
    % O1
    {
      \def\x{+2.0}
      \def\y{0.0}
      \def\radius{0.7}

      \foreach \i in {0,1,2,3}
      {
        \def\arc{-\i*360/4+45}
        \node[vertex] (O1-\i) at ({\radius*cos(\arc)+\x},{\radius*sin(\arc)+\y}) {};
      }

      \draw[edge,orangeStyle] (O1-1) -- (O1-2);
      \draw[edge,orangeStyle] (O1-3) -- (O1-0);
      \draw[edge,redStyle] (O1-0) -- (O1-1);
      \draw[edge,redStyle] (O1-2) -- (O1-3);
      \draw[edge,greenStyle] (O1-0) 
        ..controls({1.15*\radius*cos(10)+\x},{1.15*\radius*sin(10)+\y})and({1.15*\radius*cos(-10)+\x},{1.15*\radius*sin(-10)+\y}).. 
        (O1-1);
      \draw[edge,greenStyle] (O1-2) 
        ..controls({1.15*\radius*cos(190)+\x},{1.15*\radius*sin(190)+\y})and({1.15*\radius*cos(170)+\x},{1.15*\radius*sin(170)+\y}).. 
        (O1-3);
      \draw[edge,blueStyle] (O1-0) 
        ..controls({0.4*\radius*cos(10)+\x},{0.4*\radius*sin(10)+\y})and({0.4*\radius*cos(-10)+\x},{0.4*\radius*sin(-10)+\y}).. 
        (O1-1);

      \node[above=0pt of O1-3] {\small $v_1$};
      \node[below=0pt of O1-2] {\small $u_1$};

      \node at ({1.0+\x},{0.7+\y}) {\small $C_1$};
    }
  
    % O2
    {
      \def\x{+2.0}
      \def\y{-2.7}
      \def\radius{0.9}

      \foreach \i in {0,1,2,3,4,5}
      {
        \def\arc{-\i*360/6}
        \node[vertex] (O2-\i) at ({\radius*cos(\arc)+\x},{\radius*sin(\arc)+\y}) {};
      }

      \draw[edge,orangeStyle] (O2-1) -- (O2-2);
      \draw[edge,orangeStyle] (O2-3) -- (O2-4);
      \draw[edge,orangeStyle] (O2-5) -- (O2-0);
      \draw[edge,redStyle] (O2-0) -- (O2-1);
      \draw[edge,redStyle] (O2-2) -- (O2-3);
      \draw[edge,redStyle] (O2-4) -- (O2-5);
      \draw[edge,greenStyle] (O2-0) 
        ..controls({1.15*\radius*cos(-20)+\x},{1.15*\radius*sin(-20)+\y})and({1.15*\radius*cos(-40)+\x},{1.15*\radius*sin(-40)+\y}).. 
        (O2-1);
      \draw[edge,greenStyle] (O2-2) 
        ..controls({1.15*\radius*cos(-120-20)+\x},{1.15*\radius*sin(-120-20)+\y})and({1.15*\radius*cos(-120-40)+\x},{1.15*\radius*sin(-120-40)+\y}).. 
        (O2-3);
      \draw[edge,greenStyle] (O2-4) 
        ..controls({1.15*\radius*cos(-240-20)+\x},{1.15*\radius*sin(-240-20)+\y})and({1.15*\radius*cos(-240-40)+\x},{1.15*\radius*sin(-240-40)+\y}).. 
        (O2-5);
      \draw[edge,blueStyle] (O2-0)
        ..controls({0.6*\radius*cos(-20)+\x},{0.6*\radius*sin(-20)+\y})and({0.6*\radius*cos(-40)+\x},{0.6*\radius*sin(-40)+\y}).. 
        (O2-1);
      \draw[edge,blueStyle] (O2-2)
        ..controls({0.6*\radius*cos(-120-20)+\x},{0.6*\radius*sin(-120-20)+\y})and({0.6*\radius*cos(-120-40)+\x},{0.6*\radius*sin(-120-40)+\y}).. 
        (O2-3);

      \node[right=0pt of O2-5] {{\small $v_2$}};
      \node[above=0pt of O2-4] {{\small $u_2$}};

      \node at ({1.2+\x},{-0.8+\y}) {\small $C_2$};
    }

    % O3
    {
      \def\x{-1.0}
      \def\y{-3}
      \def\radius{0.9}

      \foreach \i in {0,1,2,3,4,5}
      {
        \def\arc{-\i*360/6}
        \node[vertex] (O3-\i) at ({\radius*cos(\arc)+\x},{\radius*sin(\arc)+\y}) {};
      }

      \draw[edge,orangeStyle] (O3-1) -- (O3-2);
      \draw[edge,orangeStyle] (O3-3) -- (O3-4);
      \draw[edge,orangeStyle] (O3-5) -- (O3-0);
      \draw[edge,redStyle] (O3-0) -- (O3-1);
      \draw[edge,redStyle] (O3-2) -- (O3-3);
      \draw[edge,redStyle] (O3-4) -- (O3-5);
      \draw[edge,greenStyle] (O3-0) 
        ..controls({1.15*\radius*cos(-20)+\x},{1.15*\radius*sin(-20)+\y})and({1.15*\radius*cos(-40)+\x},{1.15*\radius*sin(-40)+\y}).. 
        (O3-1);
      \draw[edge,greenStyle] (O3-2) 
        ..controls({1.15*\radius*cos(-120-20)+\x},{1.15*\radius*sin(-120-20)+\y})and({1.15*\radius*cos(-120-40)+\x},{1.15*\radius*sin(-120-40)+\y}).. 
        (O3-3);
      \draw[edge,greenStyle] (O3-4) 
        ..controls({1.15*\radius*cos(-240-20)+\x},{1.15*\radius*sin(-240-20)+\y})and({1.15*\radius*cos(-240-40)+\x},{1.15*\radius*sin(-240-40)+\y}).. 
        (O3-5);
      \draw[edge,blueStyle] (O3-0)
        ..controls({0.6*\radius*cos(-20)+\x},{0.6*\radius*sin(-20)+\y})and({0.6*\radius*cos(-40)+\x},{0.6*\radius*sin(-40)+\y}).. 
        (O3-1);
      \draw[edge,blueStyle] (O3-2)
        ..controls({0.6*\radius*cos(-120-20)+\x},{0.6*\radius*sin(-120-20)+\y})and({0.6*\radius*cos(-120-40)+\x},{0.6*\radius*sin(-120-40)+\y}).. 
        (O3-3);

      \node[above=0pt of O3-5] {{\small $v_3$}};
      \node[left=0pt of O3-4] {{\small $u_3$}};
    
      \node at ({-1.2+\x},{-0.9+\y}) {\small $C_3$};
    }

    % V^* area

    \begin{scope}
      \draw[clip,draw=none] (-2.9,2.3) rectangle (4,-4);
      \node[cloud, cloud puffs=20, draw, minimum width=6cm, minimum height=6cm] at (-2.3,2.0) {};
    \end{scope}
    \node at (-1.3,1.0) {\small{$V^*$}};

    \node[label=above:{{\small $u_0$}},vertex] (U0) at (-0.5,1.5) {};
    \node[label=left:{{\small $v_0 = v_4$}},vertex] (V0) at (-1.5,-0.1) {};
 
    % new connection

    \draw[edge,blueStyle] (U0) -- (O1-3);
    \draw[edge,blueStyle] (O1-2) -- (O2-5);
    \draw[edge,blueStyle] (O2-4) -- (O3-5);
    \draw[edge,blueStyle] (O3-4) -- (V0);
  }{}

  \def\drawCommonExchange#1#2{
    \def\x{#1}
    \def\y{#2}

    \node[vertex,label=left:{{\small $u_1$}}] (u1) at (\x-0.7,\y-0.7) {};
    \node[vertex,label=left:{{\small $u_2$}}] (u2) at (\x-0.7,\y+0.7) {};
    \node[vertex,label=above right:{{\small $v_1$}}] (v1) at (\x+0.7,\y-0.7) {};
    \node[vertex,label=below right:{{\small $v_2$}}] (v2) at (\x+0.7,\y+0.7) {};

    \draw[edge,redStyle] (u1) -- (u2) node[midway,left,black] {$e$};

    % bottom orange-blue cycle \widehat{C}
    \draw[edge,orangeStyle] (u1) ..controls(\x-0.7,\y-1)and(\x-1.1,\y-1.5).. (\x-1.1,\y-2.0);
    \draw[edge,blueStyle] (\x-1.1,\y-2.0) ..controls(\x-1.1,\y-2.3)and(\x-1.0,\y-2.7).. (\x-0.5,\y-3.0);
    \draw[edge,orangeStyle] (\x-0.5,\y-3.0) ..controls(\x-0.2,\y-3.2)and(\x+0.2,\y-3.2).. (\x+0.5,\y-3.0);
    \draw[edge,blueStyle] (\x+0.5,\y-3.0) ..controls(\x+1.0,\y-2.7)and(\x+1.1,\y-2.3).. (\x+1.1,\y-2.0);
    \draw[edge,orangeStyle] (\x+1.1,\y-2.0) ..controls(\x+1.1,\y-1.5)and(\x+0.7,\y-1).. (v1);
%    \node at (\x+0.1,\y-2.8) {$\widehat{C}$};

    % top orange-blue cycle C'
    \draw[edge,orangeStyle] (u2) ..controls(\x-1,\y+1)and(\x-1.1,\y+1.5).. (\x-1.1,\y+2.0);
    \draw[edge,blueStyle] (\x-1.1,\y+2.0) ..controls(\x-1.1,\y+2.3)and(\x-1.0,\y+2.7).. (\x-0.5,\y+3.0);
    \draw[edge,orangeStyle] (\x-0.5,\y+3.0) ..controls(\x-0.2,\y+3.2)and(\x+0.2,\y+3.2).. (\x+0.5,\y+3.0);
    \draw[edge,blueStyle] (\x+0.5,\y+3.0) ..controls(\x+1.0,\y+2.7)and(\x+1.1,\y+2.3).. (\x+1.1,\y+2.0);
    \draw[edge,orangeStyle] (\x+1.1,\y+2.0) ..controls(\x+1.1,\y+1.5)and(\x+1,\y+1).. (v2);
%    \node at (\x+0.1,\y+2.8) {$C'$};

    % red-blue cycle
    \draw[edge,redStyle] (v1) .. controls (\x+1.2,\y-0.8) .. (\x+1.3,\y-0.7);
    \draw[edge,blueStyle] (\x+1.3,\y-0.7) -- (\x+1.4,\y-0.3);
    \draw[edge,redStyle] (\x+1.4,\y-0.3) .. controls (\x+1.45,\y-0.1) and (\x+1.45,\y+0.1) .. (\x+1.4,\y+0.3);
    \draw[edge,blueStyle] (\x+1.4,\y+0.3) -- (\x+1.3,\y+0.7);
    \draw[edge,redStyle] (\x+1.3,\y+0.7) .. controls (\x+1.2,\y+0.8) .. (v2);

    % bottom right part of green-blue cycles
    \draw[edge,greenStyle] (v1) .. controls (\x+1.2,\y-1.2) .. (\x+1.4,\y-1.1);
    \draw[edge,blueStyle] (\x+1.4,\y-1.1) .. controls (\x+1.7,\y-0.9) .. (\x+1.7,\y-0.4);
    \draw[edge,greenStyle] (\x+1.7,\y-0.4) -- (\x+1.7,\y+0.5);
    \draw[edge,blueStyle] (\x+1.7,\y+0.5) .. controls (\x+1.7,\y+0.9) .. (\x+1.5,\y+1.3);
    \draw[edge,greenStyle] (\x+1.5,\y+1.3) .. controls (\x+0.9,\y+1.9) .. (\x+0.7,\y+1.8);
    \draw[edge,blueStyle] (\x+0.7,\y+1.8) .. controls (\x+0.55,\y+1.7) .. (\x+0.3,\y+1.4);

    % bottom left part of green-blue cycles
    \draw[edge,greenStyle] (u1) .. controls (\x-1.2,\y-1.3) .. (\x-1.4,\y-1.1);
    \draw[edge,blueStyle] (\x-1.4,\y-1.1) .. controls (\x-1.5,\y-0.9) .. (\x-1.5,\y-0.4);
    \draw[edge,greenStyle] (\x-1.5,\y-0.4) -- (\x-1.5,\y+0.5);
    \draw[edge,blueStyle] (\x-1.5,\y+0.5) .. controls (\x-1.5,\y+0.9) .. (\x-1.4,\y+1.3);
    \draw[edge,greenStyle] (\x-1.4,\y+1.3) .. controls (\x-0.9,\y+1.9) .. (\x-0.7,\y+1.8);
    \draw[edge,blueStyle] (\x-0.7,\y+1.8) .. controls (\x-0.55,\y+1.7) .. (\x-0.3,\y+1.4);
  }

  \piIfString{job}{ugly-exchange}{
    % middle line
    \node (divide top) at (2.1,3.5) {};
    \draw (divide top) -- (2.1,-3.5);
    \node[anchor=north east] at (divide top) {{\small $M'$}};
    \node[anchor=north west] at (divide top) {{\small $M^*$}};
  
    \drawCommonExchange{0}{0}
    \draw[edge,blueStyle] (u1) -- (v1) node[midway,above,black] {$f_1$};
    \draw[edge,blueStyle] (u2) -- (v2) node[midway,below,black] {$f_2$};
    \draw[edge,greenStyle] (0+0.3,0+1.4) .. controls (0-0.1,0+1.0) .. (u2);
    \draw[edge,greenStyle] (0-0.3,0+1.4) .. controls (0+0.1,0+1.0) .. (v2);
    \node at (0.1,-2.8) {$\widehat{C}$};
    \node at (0.1,2.8) {$C'$};

    \drawCommonExchange{+4}{0}
    \draw[edge,blueStyle] (u1) .. controls (2.2+1.35,-0.2) and (2.2+1.35,+0.2) .. (u2);
    \draw[edge,blueStyle] (v1) -- (v2);
    \draw[edge,greenStyle] (4+0.3,0+1.4) .. controls (4-0.1,0+1.0) .. (u2);
    \draw[edge,greenStyle] (4-0.3,0+1.4) .. controls (4+0.1,0+1.0) .. (v2);
  }{}

  \piIfString{job}{simple-exchange}{
    % middle line
    \node (divide top) at (2.1,3.5) {};
    \draw (divide top) -- (2.1,-3.5);
    \node[anchor=north east] at (divide top) {{\small $M'$}};
    \node[anchor=north west] at (divide top) {{\small $M^*$}};

    \drawCommonExchange{0}{0}
    \draw[edge,blueStyle] (u1) -- (v1) node[midway,above,black] {$f_1$};
    \draw[edge,blueStyle] (u2) -- (v2) node[midway,below,black] {$f_2$};
    \draw[edge,greenStyle] (0+0.3,0+1.4) .. controls (0+0.2,0+1.2) .. (v2);
    \draw[edge,greenStyle] (0-0.3,0+1.4) .. controls (0-0.2,0+1.2) .. (u2);
    \node at (0.1,-2.8) {$\widehat{C}$};
    \node at (0.1,2.8) {$C'$};

    \drawCommonExchange{+4}{0}
    \draw[edge,blueStyle] (u1) -- (v2);
    \draw[edge,blueStyle] (v1) -- (u2);
    \draw[edge,greenStyle] (4+0.3,0+1.4) .. controls (4+0.2,0+1.2) .. (v2);
    \draw[edge,greenStyle] (4-0.3,0+1.4) .. controls (4-0.2,0+1.2) .. (u2);
  }{}

  \piIfString{job}{short}{
    \def\x{0}
    \def\y{0} 

    \node[vertex,label=left:{{\small $u_1$}}] (u1) at (\x-0.7,\y-0.7) {};
    \node[vertex,label=left:{{\small $u_2$}}] (u2) at (\x-0.7,\y+0.7) {};
    \node[vertex,label=right:{{\small $v_1$}}] (v1) at (\x+0.7,\y-0.7) {};
    \node[vertex,label=right:{{\small $v_2$}}] (v2) at (\x+0.7,\y+0.7) {};

    \draw[edge,blueStyle] (u1) -- (v1) node[midway,below,black] {$f_1$};
    \draw[edge,blueStyle] (u2) -- (v2) node[midway,above,black] {$f_2$};
    \draw[edge,redStyle] (u1) -- (u2) node[midway,left,black] {$e$};
    \draw[edge,redStyle] (v1) -- (v2);
    \draw[edge,greenStyle] (u1) -- (v2);
    \draw[edge,greenStyle] (v1) -- (u2);

    % bottom orange-* cycle \widehat{C}
    \draw[edge,orangeStyle] (u1) ..controls(\x-0.7,\y-1)and(\x-1.1,\y-1.5).. (\x-1.1,\y-2.0);
    \draw[edge,blueStyle] (\x-1.1,\y-2.0) .. controls(\x-1.0,\y-2.4) .. (\x-0.5,\y-3.0);
    \draw[edge,redStyle] (\x-1.1,\y-2.0) .. controls (\x-0.6,\y-2.5) .. (\x-0.5,\y-3.0);
    \draw[edge,greenStyle] (\x-1.1,\y-2.0) .. controls(\x-1.3,\y-2.7) and (\x-1.2,\y-3.0) .. (\x-0.5,\y-3.0);
    \draw[edge,orangeStyle] (\x-0.5,\y-3.0) ..controls(\x-0.2,\y-3.2)and(\x+0.2,\y-3.2).. (\x+0.5,\y-3.0);
    \draw[edge,blueStyle] (\x+1.1,\y-2.0) .. controls(\x+1.0,\y-2.4) .. (\x+0.5,\y-3.0);
    \draw[edge,redStyle] (\x+1.1,\y-2.0) .. controls (\x+0.6,\y-2.5) .. (\x+0.5,\y-3.0);
    \draw[edge,greenStyle] (\x+1.1,\y-2.0) .. controls(\x+1.3,\y-2.7) and (\x+1.2,\y-3.0) .. (\x+0.5,\y-3.0);
    \draw[edge,orangeStyle] (\x+1.1,\y-2.0) ..controls(\x+1.1,\y-1.5)and(\x+0.7,\y-1).. (v1);
%    \node at (\x+0.1,\y-2.8) {$\widehat{C}$};

    % top orange-blue cycle C'
    \draw[edge,orangeStyle] (u2) .. controls(\x-0.7,\y+1) and (\x-1.1,\y+1.5) .. (\x-1.1,\y+2.0);
    \draw[edge,blueStyle] (\x-1.1,\y+2.0) .. controls(\x-1.0,\y+2.4) .. (\x-0.5,\y+3.0);
    \draw[edge,redStyle] (\x-1.1,\y+2.0) .. controls (\x-0.6,\y+2.5) .. (\x-0.5,\y+3.0);
    \draw[edge,greenStyle] (\x-1.1,\y+2.0) .. controls(\x-1.3,\y+2.7) and (\x-1.2,\y+3.0) .. (\x-0.5,\y+3.0);
    \draw[edge,orangeStyle] (\x-0.5,\y+3.0) ..controls(\x-0.2,\y+3.2) and (\x+0.2,\y+3.2) .. (\x+0.5,\y+3.0);
    \draw[edge,blueStyle] (\x+1.1,\y+2.0) .. controls(\x+1.0,\y+2.4) .. (\x+0.5,\y+3.0);
    \draw[edge,redStyle] (\x+1.1,\y+2.0) .. controls (\x+0.6,\y+2.5) .. (\x+0.5,\y+3.0);
    \draw[edge,greenStyle] (\x+1.1,\y+2.0) .. controls(\x+1.3,\y+2.7) and (\x+1.2,\y+3.0) .. (\x+0.5,\y+3.0);
    \draw[edge,orangeStyle] (\x+1.1,\y+2.0) ..controls(\x+1.1,\y+1.5) and (\x+0.7,\y+1) .. (v2);
%    \node at (\x+0.1,\y+2.8) {$C'$};
  }{}
}

